Towards Language Modelling in the Speech Domain Using Sub-word Linguistic Units

Language models (LMs) for text data have been studied extensively for their usefulness in language generation and other downstream tasks. However, language modelling purely in the speech domain is still a relatively unexplored topic, with traditional speech LMs often depending on auxiliary text LMs for learning distributional aspects of the language. For the English language, these LMs treat words as atomic units, which presents inherent challenges to language modelling in the speech domain. In this paper, we propose a novel LSTM-based generative speech LM that is inspired by the CBOW model and built on linguistic units including syllables and phonemes. This offers better acoustic consistency across utterances in the dataset, as opposed to single melspectrogram frames, or whole words. With a limited dataset, orders of magnitude smaller than that required by contemporary generative models, our model closely approximates babbling speech. We show the effect of training with auxiliary text LMs, multitask learning objectives, and auxiliary articulatory features. Through our experiments, we also highlight some well known, but poorly documented challenges in training generative speech LMs, including the mismatch between the supervised learning objective with which these models are trained such as Mean Squared Error (MSE), and the true objective, which is speech quality. Our experiments provide an early indication that while validation loss and Mel Cepstral Distortion (MCD) are not strongly correlated with generated speech quality, traditional text language modelling metrics like perplexity and next-token-prediction accuracy might be.

==> sections/6-results.tex <==
% Table ~\ref{tab:results1} shows the results
% of subjective and objective evaluation
% of all models. For subjective evaluation
% we report the Mean Opinion Score (MOS) and
% the results of AB testing. Evaluation is
% carried out by both the authors of the paper.
% First, we observe, as expected that our 
% proposed top-line model produces the best
% quality samples.
% % How exactly are they better?
% This is the closest approximation to babbling,
% and we find that the samples have greater 
% diversity and better prosody than those
% from other models.
% % Describe remaining results here as they
% % become available
% We find x\% agreement between both authors.

% For objective evaluation, we compare the
% generated samples against the ground truth
% examples using the Mel-Cepstral Distortion 
% (MCD).

% Our results show that while MTL and auxiliary
% text LMs both help improve the quality of 
% generated speech over the simple speech LM, 
% using ground truth articulatory Panphon features
% directly in synthesis produces the best results.


% \begin{table}[h!]
% \centering
%     \small
% \begin{tabular}{l c c}
% \toprule
% Model &  MOS & MCD \\
% \midrule
% \multicolumn{3}{c}{Syllable Level}\\
% \midrule
% Synthesis-only & 3.3 & 3.15/19.36 \\
% MTL (Panphon) & 3.4 & 3.14/19.29 \\
% Auxiliary (LSTM-LM) & 2.8 & 3.08/18.93 \\
% Auxiliary (RoBERTa) & 2.9 & 3.10/19.04 \\
% Auxiliary (Top-line) & 3.7 & 3.13/19.24 \\
% % \midrule
% % \multicolumn{3}{c}{Phoneme Level}\\
% % \midrule
% % Synthesis-only & - & - \\
% % MTL (Panphon) & - & - \\
% % Auxiliary (LSTM-LM) & - & - \\
% % Auxiliary (RoBERTa) & - & - \\
% % Auxiliary (Top-line) & - & - \\
% \bottomrule
% \end{tabular}
% \caption{Mean and standard deviation (in subscript) of quantitative measures of speech quality on 5 models
% each from syllable- and phoneme-level granularity. \label{tab:results1}}
% \end{table}

